Computing Web-scale Topic Models using an Asynchronous Parameter Server

Topic models such as Latent Dirichlet Allocation (LDA) have been widely used in information retrieval for tasks ranging from smoothing and feedback methods to tools for exploratory search and discovery. However, classical methods for inferring topic models do not scale up to the massive size of today's publicly available Web-scale data sets. The state-of-the-art approaches rely on custom strategies, implementations and hardware to facilitate their asynchronous, communication-intensive workloads. We present APS-LDA, which integrates state-of-the-art topic modeling with cluster computing frameworks such as Spark using a novel asynchronous parameter server. Advantages of this integration include convenient usage of existing data processing pipelines and eliminating the need for disk writes as data can be kept in memory from start to finish. Our goal is not to outperform highly customized implementations, but to propose a general high-performance topic modeling framework that can easily be used in today's data processing pipelines. We compare APS-LDA to the existing Spark LDA implementations and show that our system can, on a 480-core cluster, process up to 135 times more data and 10 times more topics without sacrificing model quality.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-siggraph.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-siggraph.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> sections/demo.tex <==
%!TEX root = ./../parameterserver.tex

\section*{Demo setup}

\begin{figure*}
	\centering
	\includegraphics[width=0.7\textwidth]{illustrations/demo-screenshot}
	\caption{Realtime dashboard view of the topic models being computed.}
	\label{fig:demo}
\end{figure*}

We will demonstrate the use of the Glint parameter server and the APS-LDA algorithm by running a live code example in the Spark shell that will
\begin{enumerate}
	\item Load a large dataset (100s of gigabytes) in Spark
	\item Spawn parameter servers
	\item Compute an LDA topic model in real time
\end{enumerate}

The presentation will be made possible by running a Spark shell on a remote computing cluster, where we can enter our commands in real time. Additionally, we will have a live dashboard running in a web browser that will show the computation of the LDA topic model in real time (see \cref{fig:demo}). This is accomplished by periodically polling the parameter servers for the updated parameters and displaying the top $n$ words for each topic. As a result, the audience will see a randomly initialized topic model converge to a set of coherent topics on a very large data set within just a few minutes.

The code that we will run and explain is outlined in listing \ref{lst:democode} and is concise and simple enough to be followed and understood by people with no experience in either Scala or Spark.

\subsection*{Requirements}
To make this demo possible, we require a working internet connection, either a stable WiFi signal or ethernet cable. Additionally, we require a dual screen setup, so that we can display our dashboard on one screen whilst displaying our Spark shell and code in the other. Hence, we request two displays of reasonable size (${\sim}$24").


\vfill\eject

\begin{lstlisting}[caption={Code that will run in the Spark shell.},label={lst:democode},style=scala,mathescape=true]
// 1) Load large dataset
val dataset = spark.read.format("libsvm")
       .load("./dataset.txt")

import demo.textToSparseVector
val trainingSet = dataset.map(
     x => textToSparseVector(x)
)

// 2) Start Glint parameter servers
import glint.Client
implicit val gc = Client.runOnSpark(sc)

// 3) Train an APS-LDA model
val model = new APSLDA()
   .setIterations(50)
   .setTopics(20)
   .set$\alpha$(0.05)
   .set$\beta$(0.01)
   
model.fit(trainingSet)
\end{lstlisting}



